Sparse Higher Order \v{C}ech Filtrations

For a finite set of balls of radius $r$, the $k$-fold cover is the space covered by at least $k$ balls. Fixing the ball centers and varying the radius, we obtain a nested sequence of spaces that is called the $k$-fold filtration of the centers. For $k=1$, the construction is the union-of-balls filtration that is popular in topological data analysis. For larger $k$, it yields a cleaner shape reconstruction in the presence of outliers. We contribute a sparsification algorithm to approximate the topology of the $k$-fold filtration. Our method is a combination and adaptation of several techniques from the well-studied case $k=1$, resulting in a sparsification of linear size that can be computed in expected near-linear time with respect to the number of input points. Our method also extends to the multicover bifiltration, composed of the $k$-fold filtrations for several values of $k$, with the same size and complexity bounds.

==> figures.tex <==
% This file does not compile by itself. It contains the code used for figures that are not in the main file.

%%%%% fig6 %%%%%
\tdplotsetmaincoords{65}{100}
\begin{tikzpicture}[scale=5, tdplot_main_coords, cone/.style={gray!20,opacity=0.3}]
    %standard tikz coordinate definition using x, y, z coords
	\coordinate (O) at (0,0,0);
	\coordinate (a) at (0,0,0);
    \coordinate (b) at (-0.3,0.8,0);
	
	%draw axis 
	\draw[->,black,thick] (0,-1.5,0) -- (0,-1.5,2.5) node[anchor=south]{\Huge $r$};
          	
    %<a> lenses growing
	\foreach \radius in {0,0.01,...,1}{
        %draw cone
        \tdplotdrawarc[cone]{($(a)+(0,0,\radius)$)}{\radius}{0}{360}{}{}
        \tdplotdrawarc[cone]{($(b)+(0,0,\radius)$)}{\radius}{0}{360}{}{}
	    %fill <a> lens
	    \foreach \pointa/\pointb/\cor in {a/b/blue}{
    	    \begin{scope}
                \clip ($(\pointa)+(0,0,\radius)$) circle (\radius);
        		\tdplotdrawarc[fill=\cor!60,opacity=0.3]{($(\pointb)+(0,0,\radius)$)}{\radius}{0}{360}{}{}
            \end{scope}  
        }
	}
	
	%<a> lenses frozen
	\foreach \radius in {1.01,1.02,...,1.50}{	
	    %draw cone
	    \tdplotdrawarc[cone]{($(b)+(0,0,\radius)$)}{\radius}{0}{360}{}{}
	    %fill <a> lens
	    \foreach \pointa/\pointb/\cor in {a/b/blue}{
    	    \begin{scope}
                \clip ($(\pointa)+(0,0,\radius)$) circle (1);
        		\tdplotdrawarc[fill=\cor!60,opacity=0.3]{($(\pointb)+(0,0,\radius)$)}{1}{0}{360}{}{}
            \end{scope}  
        }
        %draw cilinder
        \tdplotdrawarc[cone]{($(a)+(0,0,\radius)$)}{1}{0}{360}{}{}
	}
	
	%<a> lenses removed
	\foreach \radius in {1.50,1.51,...,1.80}{	
	    %draw cone
	    \tdplotdrawarc[cone]{($(b)+(0,0,\radius)$)}{\radius}{0}{360}{}{}
        %draw cilinder
        \tdplotdrawarc[cone]{($(a)+(0,0,\radius)$)}{1}{0}{360}{}{}
	}
\end{tikzpicture}

%%%%% 3dschematics %%%%%
\usepackage{tikz,tikz-3dplot,pgfplots} 
\usetikzlibrary{arrows,automata,positioning, shapes, shapes.geometric, calc,arrows.meta, patterns,backgrounds,intersections,angles,quotes,patterns,3d,decorations.markings,bending}
\usepackage{amsmath}
\usepgfplotslibrary{fillbetween}


\tdplotsetmaincoords{75}{-90}
\begin{tikzpicture}[scale=5, tdplot_main_coords, cone/.style={gray!30,opacity=0.3}]
    %standard tikz coordinate definition using x, y, z coords
	\coordinate (a) at (-0.5,0.8,0);
    \coordinate (b) at (0.4,0.6,0);
    \coordinate (c) at (0,0,0);
    \coordinate (d) at (-0.15,-0.5,0);	

	%draw axis 
	\draw[->,black,thick] (-1.5,1.7,0) -- (-1.5,1.7,1.8) node[anchor=south]{\Large $r$};
	%label sites
	\foreach \site in {a,b,c,d} 
        	\filldraw (\site) node[inner sep=0cm,label={[label distance=0.8pt]{180}:{\Large $\site$}}]  {} circle (0.1pt);  
          	
	%interval r=0 - r=0.4
    %all lenses grow until freeze(a)=0.4 [freeze and removal radii chosen for illustration, values are not true]
	\foreach \radius in {0,0.01,...,0.4}{
        %draw cones
        \tdplotdrawarc[cone]{($(a)+(0,0,\radius)$)}{\radius}{0}{360}{}{}
        \tdplotdrawarc[cone]{($(b)+(0,0,\radius)$)}{\radius}{0}{360}{}{}
        \tdplotdrawarc[cone]{($(c)+(0,0,\radius)$)}{\radius}{0}{360}{}{}
        \tdplotdrawarc[cone]{($(d)+(0,0,\radius)$)}{\radius}{0}{360}{}{}
	    %fill <a> lens
	    \foreach \pointa/\pointb/\cor in {a/b/blue,a/c/blue,a/d/blue}{
    	    \begin{scope}
                \clip ($(\pointa)+(0,0,\radius)$) circle (\radius);
        		\tdplotdrawarc[fill=\cor!60,opacity=0.3]{($(\pointb)+(0,0,\radius)$)}{\radius}{0}{360}{}{}
            \end{scope}  
		}
		%fill <b> lenses
	    \foreach \pointa/\pointb/\cor in {b/c/blue,b/d/red}{
    	    \begin{scope}
                \clip ($(\pointa)+(0,0,\radius)$) circle (\radius);
        		\tdplotdrawarc[fill=\cor!60,opacity=0.3]{($(\pointb)+(0,0,\radius)$)}{\radius}{0}{360}{}{}
            \end{scope}  
		}
		%fill <c> lenses
	    \foreach \pointa/\pointb/\cor in {c/d/blue}{
    	    \begin{scope}
                \clip ($(\pointa)+(0,0,\radius)$) circle (\radius);
        		\tdplotdrawarc[fill=\cor!60,opacity=0.3]{($(\pointb)+(0,0,\radius)$)}{\radius}{0}{360}{}{}
            \end{scope}  
        }
	}
	
	%interval r=0.4 - r=0.6
	%<a> lenses frozen until r=0.6, other lenses keep growing
	\foreach \radius in {0.41,0.42,...,0.60}{	
	    %draw cones
	    \tdplotdrawarc[cone]{($(b)+(0,0,\radius)$)}{\radius}{0}{360}{}{}
	    \tdplotdrawarc[cone]{($(c)+(0,0,\radius)$)}{\radius}{0}{360}{}{}
	    \tdplotdrawarc[cone]{($(d)+(0,0,\radius)$)}{\radius}{0}{360}{}{}
	    %fill <a> lenses
	    \foreach \pointa/\pointb/\cor in {a/b/blue,a/c/blue,a/d/blue}{
    	    \begin{scope}
                \clip ($(\pointa)+(0,0,\radius)$) circle (0.4);
        		\tdplotdrawarc[fill=\cor!60,opacity=0.3]{($(\pointb)+(0,0,\radius)$)}{0.4}{0}{360}{}{}
            \end{scope}  
        }
		%fill <b> lenses
	    \foreach \pointa/\pointb/\cor in {b/c/blue,b/d/red}{
    	    \begin{scope}
                \clip ($(\pointa)+(0,0,\radius)$) circle (\radius);
        		\tdplotdrawarc[fill=\cor!60,opacity=0.3]{($(\pointb)+(0,0,\radius)$)}{\radius}{0}{360}{}{}
            \end{scope}  
		}
		%fill <c> lenses
	    \foreach \pointa/\pointb/\cor in {c/d/blue}{
    	    \begin{scope}
                \clip ($(\pointa)+(0,0,\radius)$) circle (\radius);
        		\tdplotdrawarc[fill=\cor!60,opacity=0.3]{($(\pointb)+(0,0,\radius)$)}{\radius}{0}{360}{}{}
            \end{scope}  
        }
        %draw cilinder for frozen <a>
        \tdplotdrawarc[cone]{($(a)+(0,0,\radius)$)}{0.4}{0}{360}{}{}
	}
	
	%interval r=0.6 - r=0.8
	%<a> lenses removed at r=0.6, all others grow until r=0.8
	\foreach \radius in {0.61,0.62,...,0.80}{	
	    %draw cones
	    \tdplotdrawarc[cone]{($(b)+(0,0,\radius)$)}{\radius}{0}{360}{}{}
	    \tdplotdrawarc[cone]{($(c)+(0,0,\radius)$)}{\radius}{0}{360}{}{}
	    \tdplotdrawarc[cone]{($(d)+(0,0,\radius)$)}{\radius}{0}{360}{}{}
		%fill <b> lenses
	    \foreach \pointa/\pointb/\cor in {b/c/blue,b/d/red}{
    	    \begin{scope}
                \clip ($(\pointa)+(0,0,\radius)$) circle (\radius);
        		\tdplotdrawarc[fill=\cor!60,opacity=0.3]{($(\pointb)+(0,0,\radius)$)}{\radius}{0}{360}{}{}
            \end{scope}  
		}
		%fill <c> lenses
	    \foreach \pointa/\pointb/\cor in {c/d/blue}{
    	    \begin{scope}
                \clip ($(\pointa)+(0,0,\radius)$) circle (\radius);
        		\tdplotdrawarc[fill=\cor!60,opacity=0.3]{($(\pointb)+(0,0,\radius)$)}{\radius}{0}{360}{}{}
            \end{scope}  
        }
	}

	%interval r=0.8 - r=1
	%<d> lenses freeze at r=0.8, <b> and <c> lenses keep growing
	\foreach \radius in {0.81,0.82,...,1}{
        %draw cones
        \tdplotdrawarc[cone]{($(b)+(0,0,\radius)$)}{\radius}{0}{360}{}{}
        \tdplotdrawarc[cone]{($(c)+(0,0,\radius)$)}{\radius}{0}{360}{}{}
	    %fill <d> lenses
	    \foreach \pointa/\pointb/\cor/\opc in {d/b/red/0.45,d/c/blue/0.15}{
    	    \begin{scope}
                \clip ($(\pointa)+(0,0,\radius)$) circle (0.8);
        		\tdplotdrawarc[fill=\cor!60,opacity=\opc]{($(\pointb)+(0,0,\radius)$)}{0.8}{0}{360}{}{}
            \end{scope}  
        }
		%fill <b>,<c> lenses
		\foreach \pointa/\pointb/\cor in {b/c/blue}{
			\begin{scope}
				\clip ($(\pointa)+(0,0,\radius)$) circle (\radius);
				\tdplotdrawarc[fill=\cor!60,opacity=0.25]{($(\pointb)+(0,0,\radius)$)}{\radius}{0}{360}{}{}
			\end{scope}  
		}
		%draw cilinder for frozen <d>
		\tdplotdrawarc[cone]{($(d)+(0,0,\radius)$)}{0.8}{0}{360}{}{}	
	}
\end{tikzpicture}

%%%%% schematics %%%%%
\usepackage{tikz,tikz-3dplot,pgfplots} 
\usetikzlibrary{arrows,automata,positioning, shapes, shapes.geometric, calc,arrows.meta, patterns,backgrounds,intersections,angles,quotes,patterns,3d,decorations.markings,bending}
\usepackage{amsmath}

\usepgfplotslibrary{fillbetween}

\begin{tikzpicture}
    \coordinate (a) at (-0.5,0.8);
    \coordinate (b) at (0.4,0.6);
    \coordinate (c) at (0,0);
    \coordinate (d) at (-0.15,-0.5);
    
%%%%% L_r %%%%%    
    %fill intersections
    \begin{scope}
        \clip (a) circle (1);
        \foreach \site in {b,c,d} 
        \fill[gray!30] (\site) circle (1);
    \end{scope}
    \begin{scope}
        \clip (b) circle (1);
        \foreach \site in {c,d} 
        \fill[gray!30] (\site) circle (1);
    \end{scope}
    \begin{scope}
        \clip (c) circle (1);
        \foreach \site in {d} 
        \fill[gray!30] (\site) circle (1);
    \end{scope}
    %circles
    \foreach \site in {a,b,c,d} 
        \draw (\site) circle (1);
    %sites
    \filldraw (a) node[inner sep=0cm,label={[label distance=0.8pt]{0}:{$a$}}]  {} circle (1.5pt);
    \filldraw (b) node[inner sep=0cm,label={[label distance=0.8pt]{0}:{$b$}}]  {} circle (1.5pt);
    \filldraw (c) node[inner sep=0cm,label={[label distance=0.8pt]{0}:{$c$}}]  {} circle (1.5pt);
    \filldraw (d) node[inner sep=0cm,label={[label distance=0.8pt]{0}:{$d$}}]  {} circle (1.5pt);
	%label & arrow anchor
        \node[align=center] (Lr) at ($(c)+(0,-2)$) {$L_r$};    
        \node[align=center] (LrTop) at ($(c)+(0,2)$) {};
    
%%%%% U_r %%%%%
    \begin{scope}[transform canvas={xshift=4cm}]
        %fill intersections
        \begin{scope}
            \clip (b) circle (1);
            \foreach \site in {c} 
            \fill[gray!30] (\site) circle (1);
        \end{scope}
        %circles
        \foreach \site in {b,c} 
            \draw (\site) circle (1);
            \draw[dashed, gray!60] (a) circle (0.4);
            \draw[dashed, gray!60] (d) circle (0.8);
        %sites
        \filldraw (a) node[inner sep=0cm,label={[label distance=0.8pt]{0}:{$a$}}]  {} circle (1.5pt);
        \filldraw (b) node[inner sep=0cm,label={[label distance=0.8pt]{0}:{$b$}}]  {} circle (1.5pt);
        \filldraw (c) node[inner sep=0cm,label={[label distance=0.8pt]{0}:{$c$}}]  {} circle (1.5pt);
        \filldraw (d) node[inner sep=0cm,label={[label distance=0.8pt]{0}:{$d$}}]  {} circle (1.5pt);
        %label & text
        \node[align=center] (Ur) at ($(c)+(0,-2)$) {$U_r$};    
        \node[align=center] (notFilt) at ($(c)+(0,2)$) {$\{U_r\}_{r\geq 0}$ is not a filtration};    
    \end{scope}

%%%%% \tilde{L}_r %%%%%
    \begin{scope}[transform canvas={xshift=8cm}]
        %fill intersections
        \begin{scope}
            \clip (b) circle (1);
            \foreach \site in {c} 
            \fill[gray!30] (\site) circle (1);
        \end{scope}
        \begin{scope}
            \clip (d) circle (0.8);
            \foreach \site in {b,c} 
            \fill[gray!30] (\site) circle (1);
        \end{scope}
        %circles
        \foreach \site in {b,c} 
            \draw (\site) circle (1);
    	\draw (d) circle (0.8);
    	\draw[dashed, gray!60] (a) circle (0.4);
        %sites
        \filldraw (a) node[inner sep=0cm,label={[label distance=0.8pt]{0}:{$a$}}]  {} circle (1.5pt);
        \filldraw (b) node[inner sep=0cm,label={[label distance=0.8pt]{0}:{$b$}}]  {} circle (1.5pt);
        \filldraw (c) node[inner sep=0cm,label={[label distance=0.8pt]{0}:{$c$}}]  {} circle (1.5pt);
        \filldraw (d) node[inner sep=0cm,label={[label distance=0.8pt]{0}:{$d$}}]  {} circle (1.5pt);
    	%label
        \node[align=center] (tilLr) at ($(c)+(0,-2)$) {$\tilde{L}_r$};       
    \end{scope}
     
%%%%% C_r %%%%%
    \node at (0,-5) (CrFig) {\includegraphics[scale=0.25]{3dschematics.pdf}};
    \node[align=center] (Cr) at ($(c)+(0,-7)$) {$C_r$};     

%%%%% S_r %%%%%
    \begin{scope}[transform canvas={xshift=4cm,yshift=-5cm}]
    	\coordinate (ab) at (0,1);
    	\coordinate (ac) at (-0.5,0.7);
    	\coordinate (bc) at (0.4,0.5);
    	\coordinate (bd) at (0.3,0.1);
    	\coordinate (cd) at (-0.1,-0.5);
        %triangles
        \fill[gray, opacity=0.6] (ab) -- (ac) --  (bc);
        \fill[gray, opacity=0.6]  (cd) -- (bd) --  (bc);
        %edges
    	\draw[-] (ab) -- (ac) --  (bc) -- (ab);
    	\draw[-]  (cd) -- (bd) --  (bc) -- (cd);
        %vertices
        \foreach \site in {ab,ac,cd} 
        	\filldraw (\site) node[inner sep=0cm,label={[label distance=0.8pt]{160}:{$\site$}}]  {} circle (1.5pt);   
        \foreach \site in {bc,bd} 
        	\filldraw (\site) node[inner sep=0cm,label={[label distance=0.8pt]{0}:{$\site$}}]  {} circle (1.5pt);   
        %label
        \node[align=center] (Sr) at ($(c)+(0,-2)$) {$S_r$};       
    \end{scope}

%%%%% D_r %%%%%
    \begin{scope}[transform canvas={xshift=8cm,yshift=-5cm}]
        %triangles
        \fill[gray, opacity=0.6] (ab) -- (ac) --  (bc);
        \fill[gray, opacity=0.6]  (cd) -- (bd) --  (bc);
        %edges
    	\draw[-] (ab) -- (ac) --  (bc) -- (ab);
    	\draw[-]  (cd) -- (bd) --  (bc) -- (cd);
        %vertices
        \foreach \site in {ab,ac,cd} 
        	\filldraw (\site) node[inner sep=0cm,label={[label distance=0.8pt]{160}:{$\site$}}]  {} circle (1.5pt);   
        \foreach \site in {bc,bd} 
        	\filldraw (\site) node[inner sep=0cm,label={[label distance=0.8pt]{0}:{$\site$}}]  {} circle (1.5pt);   
    	%label
        \node[align=center] (Dr) at ($(c)+(0,-2)$) {$D_r$};       
    \end{scope}

%%%%% Relationships %%%%%
	\node[align=center] (tilLrTop) at ($(c)+(8,2)$) {}; 
	\node[align=center] (tilLrBottom) at ($(c)+(8,-2.3)$) {}; 
	\node[align=center] (CrTop) at ($(c)+(0,-3.5)$) {}; 
	\draw[<->,blue] (LrTop) ..controls +(up:15mm) and +(up:15mm) .. node[above] (upperText) {$(1+\epsilon)$-interleaved} (tilLrTop) ;
	\draw[<->, blue] (CrTop) ..controls +(up:15mm) and +(down:15mm) .. node[below] (middleText) {equivalent} (tilLrBottom) ;

	\node[align=center] (SrLeft) at ($(cd)+(3.5,-5.5)$) {};
	\node[align=center] (CrRight) at ($(cd)+(0.5,-5.5)$) {};
	\node[align=center] (SrRight) at ($(cd)+(4.8,-5)$) {};
	\node[align=center] (DrLeft) at ($(cd)+(7.3,-5)$) {};
	\draw[{[bend]<}-{[bend]>}, blue] (SrRight) ..controls +(down:5mm) and +(down:5mm) .. node[below] (bottonRightText) {$(1+\epsilon)$-interleaved} (DrLeft) ;                  
	\draw[{[bend]<}-{[bend]>}, blue] (CrRight) ..controls +(down:5mm) and +(down:5mm) .. node[below] (bottonLeftText) {equivalent} (SrLeft) ;            
            
\end{tikzpicture} %The freezing values were chosen only for better visualization and are not precise. 
